MIND-Stack: Modular, Interpretable, End-to-End Differentiability for Autonomous Navigation

Developing robust, efficient navigation algorithms is challenging. Rule-based methods offer interpretability and modularity but struggle with learning from large datasets, while end-to-end neural networks excel in learning but lack transparency and modularity. In this paper, we present MIND-Stack, a modular software stack consisting of a localization network and a Stanley Controller with intermediate human interpretable state representations and end-to-end differentiability. Our approach enables the upstream localization module to reduce the downstream control error, extending its role beyond state estimation. Unlike existing research on differentiable algorithms that either lack modules of the autonomous stack to span from sensor input to actuator output or real-world implementation, MIND-Stack offers both capabilities. We conduct experiments that demonstrate the ability of the localization module to reduce the downstream control loss through its end-to-end differentiability while offering better performance than state-of-the-art algorithms. We showcase sim-to-real capabilities by deploying the algorithm on a real-world embedded autonomous platform with limited computation power and demonstrate simultaneous training of both the localization and controller towards one goal. While MIND-Stack shows good results, we discuss the incorporation of additional modules from the autonomous navigation pipeline in the future, promising even greater stability and performance in the next iterations of the framework.

==> Images/Rule_vs_NE2E_vs_DiffE2e/rule_vs_ne2e_vs_diffe2e.tex <==
    \begin{enumerate}[a)]
        \item 
        \begin{tikzpicture}[font=\sffamily, thick, node distance=2.6cm, auto]
        \tikzstyle{box} = [rectangle, rounded corners, draw=Bluelight, fill=Bluelight!20, text depth=0.0cm, text width=5em, text centered, minimum height=2.0em] % Define style for boxes with rounded corners
        \tikzstyle{image node} = [rectangle]
        \node(LiDAR) {\includegraphics[width=1.5cm]{LiDARAndCamera.png}}; % Nodes
        \node[box, right of=LiDAR] (perception) {Perception};
        \node[box, right of=perception] (planning) {Planning};
        \node[box, right of=planning] (control) {Control};,
        \node[image node, right of=control] (SteerAndPedal) {\includegraphics[width=1.5cm]{SteeringWheelAndPedals.png}}
        \draw[->] (LiDAR) -- (perception); % Arrows
        \draw[->] (perception) -- (planning);
        \draw[->] (planning) -- (control);
        \draw[->] (control) -- (SteerAndPedal); 
        \end{tikzpicture}
        \item 
        \begin{tikzpicture}[yscale=0.5, xscale=1.3, every node/.style={scale=1.0}]
            % Define styles
            \tikzstyle{neuron}=[circle, draw, minimum size=10pt, inner sep=0pt]
            \tikzstyle{input neuron}=[neuron, fill=Bluelight!50];
            \tikzstyle{output neuron}=[neuron, fill=Bluelight!50];
            \tikzstyle{hidden neuron}=[neuron, fill=Bluelight!50];
            \tikzstyle{image node}=[rectangle]
        
            % Input Image Node
            \node[image node] (Input-Image) at (-2,-1.4) {\includegraphics[width=1.5cm]{LiDARAndCamera.png}};
            
            % Output Image Node
            \node[image node] (Output-Image) at (6,-1.4) {\includegraphics[width=1.5cm]{SteeringWheelAndPedals.png}};
        
            % Input layer
            \foreach \name / \y in {1,...,2}
                \node[input neuron] (I-\name) at (0,-\y) {};
        
            % Hidden layer
            \foreach \name / \y in {1,...,2}
                \node[hidden neuron] (H-\name) at (2,-\y) {};
        
            % Output layer
            \foreach \name / \y in {1,...,2}
                \node[output neuron] (O-\name) at (4,-\y) {};
        
            % Connect Image Node to first two input neurons
            \foreach \dest in {1,2}
                \draw[->] (Input-Image) -- (I-\dest);
        
            % Connect last two output neurons to Output Image Node
            \foreach \source in {1,2}
                \draw[->] (O-\source) -- (Output-Image);
        
            % Connect input layer with hidden layer
            \foreach \source in {1,...,2}
                \foreach \dest in {1,...,2}
                    \draw[->] (I-\source) -- (H-\dest);
        
            % Connect hidden layer with output layer
            \foreach \source in {1,...,2}
                \foreach \dest in {1,...,2}
                    \draw[->] (H-\source) -- (O-\dest);
        
        \end{tikzpicture}
        \item 
        \begin{tikzpicture}[font=\sffamily, thick, node distance=2.6cm, auto]
        \tikzstyle{box} = [rectangle, rounded corners, draw=Bluelight, fill=Bluelight!20, text depth=0.0cm, text width=5em, text centered, minimum height=2.0em] % Define style for boxes with rounded corners
        \tikzstyle{image node} = [rectangle]
        \node(LiDAR) {\includegraphics[width=1.5cm]{LiDARAndCamera.png}}; % Nodes
        \node[box, right of=LiDAR] (perception) {Perception};
        \node[box, right of=perception] (planning) {Planning};
        \node[box, right of=planning] (control) {Control};,
        \node[image node, right of=control] (SteerAndPedal) {\includegraphics[width=1.5cm]{SteeringWheelAndPedals.png}}
        \draw[->] (LiDAR) -- (perception); % Arrows
        \draw[->] (perception) -- (planning);
        \draw[->] (planning) -- (control);
        \draw[->] (control) -- (SteerAndPedal); 
        \draw[->, >=latex, Bluestrong, thick] (SteerAndPedal.south west) to[out=200,in=340] node[below] { \(\mathcal{L}\)} (control.south); % Feedback arrows      with labels
        \draw[->, >=latex, Bluestrong, thick] (control.south west) to[out=200,in=340] node[below] { \(\mathcal{L}\)} (planning.south);
        \draw[->, >=latex, Bluestrong, thick] (planning.south west) to[out=200,in=340] node[below] { \(\mathcal{L}\)} (perception.south);
        \end{tikzpicture}

        % Subplot 2
        \begin{tikzpicture}[font=\sffamily, thick, node distance=2.6cm, auto]
            % Define styles
            \tikzstyle{box} = [rectangle, rounded corners, draw=Bluelight, fill=Bluelight!20, text depth=0.0cm, text width=5em, text centered, minimum height=2.0em]
            \tikzstyle{invisable box} = [rectangle, rounded corners, text depth=0.0cm, text width=5em, text centered, minimum height=2.0em]
            \tikzstyle{neuron} = [circle, draw, fill=orange!50, minimum size=4mm] % Adjusted size for visibility
        
            % Nodes
            \node (LiDAR) {\includegraphics[width=1.5cm]{LiDARAndCamera.png}};
            \node[box, right of=LiDAR] (perception) {Perception};
        
            % Neural Network Planning Nodes
            \node[invisable box, right of=perception] (NN) {}; % This node is just for positioning reference
            \node[neuron, above right=-0.2cm and 1.5cm of perception] (N-1) {}; % Adjusted for better vertical positioning
            \node[neuron, below right=-0.2cm and 1.5cm of perception] (N-2) {}; % Adjusted for better vertical positioning
        
            \node[box, right of=NN] (control) {Control};
            \node[right of=control] (SteerAndPedal) {\includegraphics[width=1.5cm]{SteeringWheelAndPedals.png}};
        
            % Arrows
            \draw[->] (LiDAR) -- (perception);
            \foreach \y in {1,2}
                \draw[->] (perception) -- (N-\y); % Connect perception to each neuron
            \foreach \y in {1,2}
                \draw[->] (N-\y) -- (control); % Connect each neuron to control
            \draw[->] (control) -- (SteerAndPedal);
        
            % Feedback arrows with labels
            \draw[->, >=latex, thick, Bluestrong] (SteerAndPedal.south west) to[out=200,in=340] node[below] { \(\mathcal{L}\)} (control.south);
            \draw[->, >=latex, thick, Bluestrong] (control.south west) to[out=200,in=340] node[below] { \(\mathcal{L}\)} (N-2.south);
            \draw[->, >=latex, thick, Bluestrong] (N-2.south west) to[out=200,in=340] node[below] { \(\mathcal{L}\)} (perception.south);
        
        \end{tikzpicture}

        
    \end{enumerate}

==> Images/rule_vs_network_vs_differential/rule_vs_network_vs_differential.tex <==
\begin{tikzpicture}

% Define styles
\tikzstyle{module} = [rectangle, draw=blue, thick, rounded corners, fill=blue!20, text width=1.5cm, align=center, minimum height=0.5cm, rotate=90]

% Standard Stack
\node at (-3.5, 2) [text width=2.5cm, align=center] {\textbf{Standard Stack}};
\node (perception) at (-4, 0) [module] {Perception};
\node (prediction) at (-3, 0) [module] {Prediction};
\node (planning) at (-2, 0) [module] {Planning};
\node (control) at (-1, 0) [module] {Control};

\draw[blue, thick, rounded corners] (-4.5, -1.5) rectangle (-0.5, 1.5);

% Plus sign
\node at (0, 0) {\Huge +};

% Differentiable Policy
\node at (2, 2) [text width=2.5cm, align=center] {\textbf{Differentiable Policy}};
\draw[blue, thick] (1.5, -1) -- (2.5, 1);
\draw[blue, thick] (1.5, 1) -- (2.5, -1);
\draw[blue, thick] (2, -1.5) -- (2, 1.5);
\draw[blue, thick] (1.5, -1) -- (2.5, -1);
\draw[blue, thick] (1.5, 1) -- (2.5, 1);
\draw[blue, thick] (1.5, -1) -- (1.5, 1);
\draw[blue, thick] (2.5, -1) -- (2.5, 1);
\foreach \x in {1.7, 1.9, 2.1, 2.3} {
    \foreach \y in {-0.8, -0.4, 0, 0.4, 0.8} {
        \node[draw=blue, circle, fill=white, minimum size=3pt, inner sep=0pt] at (\x, \y) {};
    }
}

% Equals sign
\node at (3, 0) {\Huge =};

% Differentiable Stack
\node at (5, 2) [text width=2.5cm, align=center] {\textbf{Differentiable Stack}};
\node (d_perception) at (4, 0) [module] {Perception};
\node (d_prediction) at (5, 0) [module] {Prediction};
\node (d_planning) at (6, 0) [module] {Planning};
\node (d_control) at (7, 0) [module] {Control};

\draw[blue, thick, rounded corners] (3.5, -1.5) rectangle (7.5, 1.5);

% Connections
\foreach \y in {-0.6, 0, 0.6} {
    \foreach \x in {3.8, 4.8, 5.8, 6.8} {
        \node[draw=blue, circle, fill=white, minimum size=3pt, inner sep=0pt] at (\x, \y) {};
    }
    \draw[blue, thick] (3.8, \y) -- (4.8, \y);
    \draw[blue, thick] (4.8, \y) -- (5.8, \y);
    \draw[blue, thick] (5.8, \y) -- (6.8, \y);
    \draw[blue, thick] (6.8, \y) -- (7.8, \y);
}

\end{tikzpicture}


==> Images/stack_structure/stack_structure.tex <==
\begin{tikzpicture}

% Define styles
\tikzstyle{module} = [rectangle, draw=blue, thick, rounded corners, fill=blue!20, text width=1.5cm, align=center, minimum height=0.5cm, rotate=90]
\tikzstyle{module_nn} = [rectangle, draw=blue, thick, rounded corners, fill=blue!20, text width=2.5cm, align=center, minimum height=0.5cm, rotate=90]

% Standard Stack
\node at (-3.5, 2.5) [text width=2.5cm, align=center] {\textbf{Standard Stack}};
\node (perception) at (-4, 0) [module] {Perception};
\node (prediction) at (-3, 0) [module] {Prediction};
\node (planning) at (-2, 0) [module] {Planning};
\node (control) at (-1, 0) [module] {Control};

\draw[blue, thick, rounded corners] (-4.5, -1.5) rectangle (-0.5, 1.5);

% Plus sign
\node at (0, 0) {\Huge +};

% Differentiable Policy
\node at (2.5, 2.5) [text width=2.5cm, align=center] {\textbf{Differentiable Policy}};
\draw[blue, thick] (1.5, -1) -- (3.5, 1);
\draw[blue, thick] (1.5, 1) -- (3.5, -1);
\draw[blue, thick] (2.5, -1.5) -- (2.5, 1.5);
\draw[blue, thick] (1.5, -1) -- (3.5, -1);
\draw[blue, thick] (1.5, 1) -- (3.5, 1);
\draw[blue, thick] (1.5, -1) -- (1.5, 1);
\draw[blue, thick] (3.5, -1) -- (3.5, 1);
\foreach \x in {1.8, 2.2, 2.5, 2.8, 3.2} {
    \foreach \y in {-0.8, -0.4, 0, 0.4, 0.8} {
        \node[draw=blue, circle, fill=white, minimum size=3pt, inner sep=0pt] at (\x, \y) {};
    }
}

% Equals sign
\node at (4.5, 0) {\Huge =};

% Differentiable Stack
\node at (7, 2.5) [text width=2.5cm, align=center] {\textbf{Differentiable Stack}};
\node (d_perception) at (6, 0) [module_nn] {Perception};
\node (d_prediction) at (7.5, 0) [module_nn] {Prediction};
\node (d_planning) at (9, 0) [module_nn] {Planning};
\node (d_control) at (10.5, 0) [module_nn] {Control};

\draw[blue, thick, rounded corners] (5.5, -1.5) rectangle (11, 1.5);

% Neural Network Connections for Differentiable Stack
\foreach \y in {-0.6, 0, 0.6} {
    \foreach \x in {5.8, 7.3, 8.8, 10.3} {
        \node[draw=blue, circle, fill=white, minimum size=3pt, inner sep=0pt] at (\x, \y) {};
    }
    \draw[blue, thick] (5.8, \y) -- (7.3, \y);
    \draw[blue, thick] (7.3, \y) -- (8.8, \y);
    \draw[blue, thick] (8.8, \y) -- (10.3, \y);
    \draw[blue, thick] (10.3, \y) -- (11.8, \y);
}

\end{tikzpicture}

==> Plots/Real_Vehicle_Heading_Error/real_vehicle_heading_error.tex <==

    \begin{tikzpicture}
        \begin{axis}[
            width=1.0\textwidth, % Scale the plot width
            height=0.85\textwidth, % Scale the plot height
            xlabel={Training Lap},
            ylabel={Heading Error \(e_{\text{head}}\) in \unit{rad}},
            xmin=0, xmax=22,
            ymin=110, ymax=140,
            xtick={0,5,10,15,20},
            ytick={110,120,130,140},
            grid=major,
            grid style={lightgray!50},
            legend pos=north east,
            legend style={draw=none, cells={align=left}},
            every axis plot/.append style={thick},
            tick align=outside,
            enlargelimits=false
        ]
        \addplot[
            color=Bluelight,
            mark=*,
            mark options={fill=Bluelight},
            line width=0.75pt,
            mark size=2pt,
            nodes near coords,
            point meta=explicit symbolic
        ] table [x=Lap, y=Error, col sep=comma] {
            Lap,Error
            1,134.0146
            2,131.0571
            3,132.3453
            4,131.6929
            5,133.8808
            6,128.6555
            7,127.1894
            8,123.5301
            9,125.3576
            10,128.0565
            11,125.8879
            12,121.9873
            13,123.3783
            14,128.9668
            15,124.4710
            16,121.5176
            17,126.2413
            18,125.5631
            19,122.7010
            20,127.5900
            21,115.3796
            22,117.4826
        };

        \legend{GT Heading Error \\ per lap}
        \end{axis}
    \end{tikzpicture}
    

==> Plots/Sim_Crosstrack_Loss/sim_crosstrack_loss_gt.tex <==

    \begin{tikzpicture}
        \begin{axis}[
            width=1.0\textwidth, % Scale the plot width
            height=0.68\textwidth, % Scale the plot height
            xlabel={Training Lap},
            ylabel={Abs. GT CTE \(e_{\text{cross-gt}}\) in \unit{m}},
            xmin=0, xmax=30,
            ymin=108, ymax=140,
            xtick={0,10,20,30},
            ytick={140, 130, 120, 110},
            grid=major,
            grid style={lightgray!50},
            legend pos=north east,
            legend style={draw=none, cells={align=left}},
            every axis plot/.append style={thick},
            tick align=outside,
            enlargelimits=false
        ]
        \addplot[
            color=Bluelight,
            mark=*,
            mark options={fill=Bluelight},
            line width=0.75pt,
            mark size=2pt,
            nodes near coords,
            point meta=explicit symbolic
        ] table [x=Step, y=Value, col sep=comma] {Plots/Sim_Crosstrack_Loss/20_8_gt.csv};

        \legend{Abs. GT \\ Crosstrack \\ Error per lap}
        \end{axis}
    \end{tikzpicture}
    \caption{Reduction in ground truth crosstrack error achieved by the MIND-Stack.}
    \label{fig:crosstrack_gt_error}

==> Plots/Sim_Crosstrack_Loss/sim_crosstrack_loss_sae.tex <==

    \begin{tikzpicture}
        \begin{axis}[
            width=0.4\textwidth, % Scale the plot width
            height=0.25\textwidth, % Scale the plot height
            xlabel={Training Lap},
            ylabel={Sq. CTE \(e^2_{\text{cross}}\) in \unit{m^2}},
            xmin=0, xmax=30,
            ymin=0, ymax=102,
            xtick={0,10,20,30},
            ytick={0,20,40, 60,80,100},
            grid=major,
            grid style={lightgray!50},
            legend pos=north east,
            legend style={draw=none, cells={align=left}},
            every axis plot/.append style={thick},
            tick align=outside,
            enlargelimits=false
        ]
        \addplot[
            color=Bluelight,
            mark=*,
            mark options={fill=Bluelight},
            line width=0.75pt,
            mark size=2pt,
            nodes near coords,
            point meta=explicit symbolic
        ] table [x=Step, y=Value, col sep=comma] {Plots/Sim_Heading_Loss_Squared/0.0_5.5_0.0_0.0_4e-08_Time_ 2024-08-11_16-17-49.csv};

        \legend{Sq. Crosstrack \\ Error per lap}
        \end{axis}
    \end{tikzpicture}
    \caption{Training the localization module to minimize the control error in Scenario 2, shows a clear \textbf{reduction in the control loss}.}
    \label{fig:crosstrack_error}

==> Plots/Sim_Heading_Loss/sim_heading_loss_single.tex <==

    \begin{tikzpicture}
        \begin{axis}[
            width=1.0\textwidth, % Scale the plot width
            height=0.65\textwidth, % Scale the plot height
            xlabel={Training Lap},
            ylabel={HE \(e_{\text{head}}\) in \unit{rad}},
            xmin=0, xmax=30,
            ymin=-34, ymax=4,
            xtick={0,10,20,30},
            ytick={-30,-20,-10,0},
            grid=major,
            grid style={lightgray!50},
            legend pos=north west,
            legend style={draw=none, cells={align=left}},
            every axis plot/.append style={thick},
            tick align=outside,
            enlargelimits=false
        ]
        \addplot[
            color=Bluelight,
            mark=*,
            mark options={fill=Bluelight},
            line width=0.75pt,
            mark size=2pt,
            nodes near coords,
            point meta=explicit symbolic
        ] table [x=Step, y=Value, col sep=comma] {Plots/Sim_Heading_Loss/16_17_error.csv};

        \legend{Heading Error \\ per lap}
        \end{axis}
    \end{tikzpicture}
    \caption{Training the localization module to minimize the control heading error.}
    \label{fig:heading_single_error}

==> Plots/Sim_Heading_Loss/sim_heading_loss_single_gt.tex <==

    \begin{tikzpicture}
        \begin{axis}[
            width=1.0\textwidth, % Scale the plot width
            height=0.65\textwidth, % Scale the plot height
            xlabel={Training Lap},
            ylabel={GT HE \(e_{\text{head-gt}}\) in \unit{rad}},
            xmin=0, xmax=30,
            ymin=20, ymax=27,
            xtick={0,10,20,30},
            ytick={20,21,22,23, 24, 25, 26, 27},
            grid=major,
            grid style={lightgray!50},
            legend pos=south west,
            legend style={draw=none, cells={align=right}},
            every axis plot/.append style={thick},
            tick align=outside,
            enlargelimits=false
        ]
        \addplot[
            color=Bluelight,
            mark=*,
            mark options={fill=Bluelight},
            line width=0.75pt,
            mark size=2pt,
            nodes near coords,
            point meta=explicit symbolic
        ] table [x=Step, y=Value, col sep=comma] {Plots/Sim_Heading_Loss/16_17_gt.csv};

        \legend{GT Heading \\ Error per lap}
        \end{axis}
    \end{tikzpicture}
    \caption{Improvement in ground truth heading error achieved by the MIND-Stack.}
    \label{fig:heading_single_gt_error}

==> Plots/Sim_Heading_Loss_Squared/sim_heading_loss_squared_gt.tex <==
\begin{tikzpicture}
        \begin{axis}[
            width=1.0\textwidth, % Scale the plot width
            height=0.73\textwidth, % Scale the plot height
            xlabel={Training Lap},
            ylabel={GT HE \(e_{\text{headgt}}\) in \(rad\)},
            xmin=0, xmax=30,
            ymin=24, ymax=28,
            xtick={0,10,20,30},
            ytick={24,25,26,27,28},
            grid=major,
            grid style={lightgray!50},
            legend pos=north east,
            legend style={draw=none, cells={align=left}},
            every axis plot/.append style={thick},
            tick align=outside,
            enlargelimits=false
        ]
        \addplot[
            color=Bluelight,
            mark=*,
            mark options={fill=Bluelight},
            line width=0.75pt,
            mark size=2pt,
            nodes near coords,
            point meta=explicit symbolic
        ] table [x=Step, y=Value, col sep=comma] {Plots/Sim_Heading_Loss_Squared/16_17_gt.csv};

        \legend{GT Heading Error per lap}
        \end{axis}
    \end{tikzpicture}
    \caption{XYZ.}
    \label{fig:heading_squared_gt_error}

==> Plots/Sim_Heading_Loss_Squared/sim_heading_loss_squared_smaller.tex <==

    \begin{tikzpicture}
        \begin{axis}[
            width=1.0\textwidth, % Scale the plot width
            height=0.7\textwidth, % Scale the plot height
            xlabel={Training Lap},
            xmin=0, xmax=30,
            ymin=30, ymax=70,
            xtick={0,10,20,30},
            ytick={30,40,50,60,70},
            grid=major,
            grid style={lightgray!50},
            legend pos=north east,
            legend style={draw=none, cells={align=left}},
            every axis plot/.append style={thick},
            tick align=outside,
            enlargelimits=false
        ]
        \addplot[
            color=Bluelight,
            mark=*,
            mark options={fill=Bluelight},
            line width=0.75pt,
            mark size=2pt,
            nodes near coords,
            point meta=explicit symbolic
        ] table [x=Step, y=Value, col sep=comma] {Plots/Sim_Heading_Loss_Squared/16_17.csv};

        \legend{Squared Heading \\ Error per lap in \unit{rad^2}}
        \end{axis}
    \end{tikzpicture}
    \caption{Training the localization module to minimize the control squared heading error.}
    \label{fig:squared_heading_error}
